Cross-Modal Distillation for RGB-Depth Person Re-Identification

Person re-identification is a key challenge for surveillance across multiple sensors. Prompted by the advent of powerful deep learning models for visual recognition, and inexpensive RGB-D cameras and sensor-rich mobile robotic platforms, e.g. self-driving vehicles, we investigate the relatively unexplored problem of cross-modal re-identification of persons between RGB (color) and depth images. The considerable divergence in data distributions across different sensor modalities introduces additional challenges to the typical difficulties like distinct viewpoints, occlusions, and pose and illumination variation. While some work has investigated re-identification across RGB and infrared, we take inspiration from successes in transfer learning from RGB to depth in object detection tasks. Our main contribution is a novel method for cross-modal distillation for robust person re-identification, which learns a shared feature representation space of person's appearance in both RGB and depth images. In addition, we propose a cross-modal attention mechanism where the gating signal from one modality can dynamically activate the most discriminant CNN filters of the other modality. The proposed distillation method is compared to conventional and deep learning approaches proposed for other cross-domain re-identification tasks. Results obtained on the public BIWI and RobotPKU datasets indicate that the proposed method can significantly outperform the state-of-the-art approaches by up to 16.1% in mean Average Precision (mAP), demonstrating the benefit of the distillation paradigm. The experimental results also indicate that using cross-modal attention allows to improve recognition accuracy considerably with respect to the proposed distillation method and relevant state-of-the-art approaches.

==> table_atten_biwi.tex <==
\begin{table*}[t!]

\caption{Average accuracy of proposed network with attention for different scenarios on the BIWI dataset.
}
\resizebox{\linewidth}{!}
{\begin{tabular}{|l||l|l|l|l||l|l|l|l|}
\hline
{\textbf{Approach}}      & \multicolumn{4}{l||}{\textbf{Query-RGB, Gallery-Depth}}                     & \multicolumn{4}{l|}{\textbf{Query-Depth, Gallery-RGB}}                     \\ \cline{2-9} 
                                        & \textbf{rank-1 (\%)} & \textbf{rank-5 (\%)} & \textbf{rank-10 (\%)} & \textbf{mAP (\%)} & \textbf{rank-1 (\%)} & \textbf{rank-5 (\%)} & \textbf{rank-10 (\%)} & \textbf{mAP (\%)} \\ \hline \hline
             
\begin{tabular}[c]{@{}l@{}} Cross-modal distillation network (ours)\end{tabular}& 32.6 $\pm$ 1.6  & 70.9 $\pm$ 0.2  & 88.8 $\pm$ 0.8  & 33.0 $\pm$ 1.8  & 36.6 $\pm$ 0.7  & 76.7 $\pm$ 1.1  & 92.3 $\pm$ 1.9  & 38.4 $\pm$ 1.7    \\ \hline


\begin{tabular}[c]{@{}l@{}}\textbf{Cross-modal distillation network + Attention (ours)}\end{tabular}& \textbf{40.4 $\pm$ 2.1}  & \textbf{77.1 $\pm$ 1.7}  & \textbf{91.0 $\pm$ 1.0}  & \textbf{41.3 $\pm$ 1.8}  & \textbf{42.8 $\pm$ 3.9}  & \textbf{80.3 $\pm$ 1.6}  & \textbf{93.5 $\pm$ 1.0}  & \textbf{43.9 $\pm$ 3.9}    \\ \hline
\end{tabular}}
\label{attnbiwi}
\end{table*}

==> table_atten_pku.tex <==
\begin{table*}[t!]
\caption{Average accuracy of state-of-the-art and proposed architecture for different scenarios on the RobotPKU dataset.}
\resizebox{\linewidth}{!}
{\begin{tabular}{|l||l|l|l|l||l|l|l|l|}
\hline
{\textbf{Approach}}      & \multicolumn{4}{l||}{\textbf{Query-RGB, Gallery-Depth}}                     & \multicolumn{4}{l|}{\textbf{Query-Depth, Gallery-RGB}}                     \\ \cline{2-9} 
                                        & \textbf{rank-1 (\%)} & \textbf{rank-5 (\%)} & \textbf{rank-10 (\%)} & \textbf{mAP (\%)} & \textbf{rank-1 (\%)} & \textbf{rank-5 (\%)} & \textbf{rank-10 (\%)} & \textbf{mAP (\%)} \\ \hline \hline


\begin{tabular}[c]{@{}l@{}}\textbf{Cross-modal distillation network (ours)}\end{tabular}&  19.5 $\pm$ 1.0  & 50.1 $\pm$ 0.5  & 67.9 $\pm$ 0.7  & 18.1 $\pm$ 1.2 & 21.5 $\pm$ 1.1 & 54.9 $\pm$ 1.4  & 72.6 $\pm$ 1.0  & 20.5 $\pm$ 1.0    \\ \hline

\begin{tabular}[c]{@{}l@{}}\textbf{Cross-modal distillation network + Attention (ours)}\end{tabular}&  \textbf{25.3 $\pm$ 2.0}  & \textbf{58.1 $\pm$ 2.5}  & \textbf{74.7 $\pm$ 1.7}  &\textbf{23.5 $\pm$ 2.0}          & \textbf{22.9 $\pm$ 1.8}  & \textbf{56.0 $\pm$ 2.0}  & \textbf{72.8 $\pm$ 1.8}  & \textbf{22.4 $\pm$ 1.9}    \\ \hline

\end{tabular}}
\label{attnpku}
\end{table*}
